A Framework for In-Vivo Testing of Mobile Applications

The ecosystem in which mobile applications run is highly heterogeneous and configurable. All layers upon which mobile apps are built offer wide possibilities of variations, from the device and the hardware, to the operating system and middleware, up to the user preferences and settings. Testing all possible configurations exhaustively, before releasing the app, is unaffordable. As a consequence, the app may exhibit different, including faulty, behaviours when executed in the field, under specific configurations. In this paper, we describe a framework that can be instantiated to support in-vivo testing of a mobile app. The framework monitors the configuration in the field and triggers in-vivo testing when an untested configuration is recognized. Experimental results show that the overhead introduced by monitoring is unnoticeable to negligible (i.e., 0-6%) depending on the device being used (high- vs. low-end). In-vivo test execution required on average 3s: if performed upon screen lock activation, it introduces just a slight delay before locking the device.

==> tabs/tab.pref.tex <==
% latex table generated in R 3.5.2 by xtable 1.8-4 package
% Tue Oct  8 10:24:20 2019
\begin{table}[ht]
\centering
\caption{Mapping of app preferences to feature model. Column \emph{Total} shows the total number of preferences in the app, columns \emph{Direct}, \emph{Heuristics}, \emph{Unsup} show, respectively, the percentage of preferences directly mapped to feature model elements, mapped by applying custom heuristics, and those currently unsupported by the automated analysis of VATE. Apps used in RQ2 are shown in \textbf{boldface}.} 
\label{tab:pref2fm}
{\scriptsize
\begin{tabular}{rlrrrr}
  \hline
 & \textbf{App} & \textbf{Total} & \textbf{Direct(\%)} & \textbf{Heuristics(\%)} & \textbf{Unsup(\%)} \\ 
  \hline
1 & A2dpvol &  15 & 100.00 & 0.00 & 0.00 \\ 
  2 & Forecastie &  15 & 86.67 & 13.33 & 0.00 \\ 
  3 & Hackernews &   6 & 100.00 & 0.00 & 0.00 \\ 
  4 & Nanoconverter &  42 & 100.00 & 0.00 & 0.00 \\ 
  5 & Notepad &   7 & 100.00 & 0.00 & 0.00 \\ 
  6 & Connectbot &  23 & 91.30 & 4.35 & 4.35 \\ 
  7 & RedReader &  74 & 93.24 & 1.35 & 5.41 \\ 
  8 & Wikipedia &  58 & 53.45 & 36.21 & 10.34 \\ 
  9 & Runnerup &  78 & 66.67 & 19.23 & 14.10 \\ 
  10 & Suntimes &  28 & 82.14 & 0.00 & 17.86 \\ 
  11 & KISS &  48 & 70.83 & 2.08 & 27.08 \\ 
  12 & Commons &   7 & 57.14 & 14.29 & 28.57 \\ 
  13 & Alwayson &  40 & 70.00 & 0.00 & 30.00 \\ 
  14 & Amaze &  47 & 61.70 & 4.26 & 34.04 \\ 
  15 & Gw &  17 & 64.71 & 0.00 & 35.29 \\ 
  16 & Radiocells &  28 & 42.86 & 21.43 & 35.71 \\ 
  17 & TintBrowser &  33 & 51.52 & 9.09 & 39.39 \\ 
  18 & AnkiDroid & 122 & 52.46 & 5.74 & 41.80 \\ 
  19 & Uhabits &  19 & 47.37 & 10.53 & 42.11 \\ 
  20 & Vanilla &  42 & 57.14 & 0.00 & 42.86 \\ 
  21 & Aphotomanager &  29 & 51.72 & 3.45 & 44.83 \\ 
  22 & OmniNotes &  40 & 50.00 & 5.00 & 45.00 \\ 
  23 & Opensudoku &  26 & 53.85 & 0.00 & 46.15 \\ 
  24 & Timber &  17 & 52.94 & 0.00 & 47.06 \\ 
  25 & Signal &  76 & 50.00 & 1.32 & 48.68 \\ 
  26 & OpenBikeSharing &   8 & 37.50 & 12.50 & 50.00 \\ 
  27 & Antennapod &  69 & 49.28 & 0.00 & 50.72 \\ 
  28 & Materialistic &  43 & 44.19 & 2.33 & 53.49 \\ 
  29 & Ammx &  63 & 39.68 & 3.17 & 57.14 \\ 
  30 & Fillup &  12 & 41.67 & 0.00 & 58.33 \\ 
   \hline
\end{tabular}
}
\end{table}


==> tabs/tab.rq2.results.cpusum.tex <==
\begin{table*}[htb]
\centering
\caption{Results of the measurement in Firebase test-lab. Clean and \tool columns contain the amount of resources (CPU, memory and network) usage, the $\Delta\%$ column contains the percentage of overhead introduced by \tool and the \#sig column is the number of scenarios whose P-value is less than 0.05 (out of 4 scenarios)}
\label{table:rq2-results}
\begin{tabular}{ll|rrrr|rrrr|rrrrr}
\hline
&  & 
\multicolumn{4}{c|}{\textbf{CPU ($\Sigma\%$)}} & 
\multicolumn{4}{c|}{\textbf{Memory (MB)}} & 
\multicolumn{5}{c}{\textbf{Network (KB)}} \\
\textbf{App} & \textbf{Device} & 
\textbf{Clean} & \textbf{\tool} & \textbf{$\Delta\%$} & \textbf{\#sig} &
\textbf{Clean} & \textbf{\tool} & \textbf{$\Delta\%$} & \textbf{\#sig} &
\textbf{Clean} & \textbf{\tool} & \textbf{$\Delta$} & \textbf{$\Delta\%$} & \textbf{\#sig} \\
\hline
Amaze & moto-e5-play & 339.2 & 352.5 & 3.9 & 3 & 49.2 & 49.8 & 1.4 & 4 & 3.2 & 9.2 & 6.0 & 188.4 & 3 \\ 
   & google-pixel2 & 81.5 & 84.2 & 3.3 & 3 & 105.8 & 106.1 & 0.3 & 1 & 3.6 & 8.9 & 5.3 & 146.0 & 3 \\ 
   & oneplus-6t & 65.3 & 67.4 & 3.2 & 3 & 113.5 & 114.2 & 0.6 & 0 & 2.0 & 4.8 & 2.8 & 136.5 & 4 \\ 
\hline
  Forecastie & moto-e5-play & 241.5 & 246.2 & 2.0 & 3 & 29.7 & 29.8 & 0.4 & 3 & 92.1 & 96.8 & 4.7 & 5.1 & 2 \\ 
   & google-pixel2 & 54.9 & 56.4 & 2.8 & 2 & 63.5 & 63.7 & 0.3 & 0 & 95.5 & 99.2 & 3.7 & 3.9 & 1 \\ 
   & oneplus-6t & 48.1 & 48.9 & 1.7 & 0 & 72.6 & 72.8 & 0.3 & 1 & 92.9 & 93.2 & 0.3 & 0.3 & 1 \\ 
\hline
  Materialistic & moto-e5-play & 555.6 & 535.6 & -3.6 & 0 & 50.6 & 48.9 & -3.4 & 0 & 2499.5 & 2065.5 & -434.0 & -17.4 & 0 \\ 
   & google-pixel2 & 126.6 & 125.4 & -1.0 & 0 & 107.6 & 102.4 & -4.9 & 1 & 2992.5 & 2873.8 & -118.7 & -4.0 & 0 \\ 
   & oneplus-6t & 114.8 & 109.2 & -4.9 & 0 & 122.1 & 113.3 & -7.2 & 0 & 3213.6 & 2919.7 & -293.9 & -9.1 & 0 \\ 
\hline
  Redreader & moto-e5-play & 737.4 & 752.8 & 2.1 & 0 & 37.5 & 37.9 & 1.0 & 2 & 24154.9 & 23130.3 & -1024.6 & -4.2 & 0 \\ 
   & google-pixel2 & 160.8 & 163.9 & 1.9 & 0 & 75.3 & 76.4 & 1.4 & 2 & 32940.5 & 32645.2 & -295.3 & -0.9 & 0 \\ 
   & oneplus-6t & 145.0 & 147.2 & 1.5 & 0 & 83.7 & 84.8 & 1.3 & 3 & 33384.9 & 30707.9 & -2677.0 & -8.0 & 0 \\ 
\hline
  Timber & moto-e5-play & 245.3 & 250.1 & 2.0 & 2 & 44.5 & 43.6 & -2.1 & 0 & 23.6 & 26.9 & 3.3 & 14.1 & 2 \\ 
   & google-pixel2 & 66.1 & 66.6 & 0.8 & 0 & 87.5 & 88.5 & 1.2 & 3 & 30.1 & 31.5 & 1.3 & 4.4 & 1 \\ 
   & oneplus-6t & 55.5 & 57.0 & 2.6 & 1 & 104.4 & 105.0 & 0.5 & 1 & 18.6 & 20.4 & 1.8 & 9.7 & 3 \\ 
\hline
  Uhabits & google-pixel2 & 48.4 & 48.5 & 0.2 & 1 & 70.3 & 71.2 & 1.3 & 4 & 0.3 & 4.4 & 4.0 & 1295.0 & 4 \\ 
   & oneplus-6t & 39.8 & 39.8 & -0.0 & 0 & 76.5 & 76.6 & 0.1 & 1 & 0.0 & 2.7 & 2.7 & -- & 4 \\ 
\hline
\end{tabular}
\end{table*}

